Gotta Catch 'Em All: Using Honeypots to Catch Adversarial Attacks on Neural Networks

Deep neural networks (DNN) are known to be vulnerable to adversarial attacks. Numerous efforts either try to patch weaknesses in trained models, or try to make it difficult or costly to compute adversarial examples that exploit them. In our work, we explore a new "honeypot" approach to protect DNN models. We intentionally inject trapdoors, honeypot weaknesses in the classification manifold that attract attackers searching for adversarial examples. Attackers' optimization algorithms gravitate towards trapdoors, leading them to produce attacks similar to trapdoors in the feature space. Our defense then identifies attacks by comparing neuron activation signatures of inputs to those of trapdoors. In this paper, we introduce trapdoors and describe an implementation of a trapdoor-enabled defense. First, we analytically prove that trapdoors shape the computation of adversarial attacks so that attack inputs will have feature representations very similar to those of trapdoors. Second, we experimentally show that trapdoor-protected models can detect, with high accuracy, adversarial examples generated by state-of-the-art attacks (PGD, optimization-based CW, Elastic Net, BPDA), with negligible impact on normal classification. These results generalize across classification domains, including image, facial, and traffic-sign recognition. We also present significant results measuring trapdoors' robustness against customized adaptive attacks (countermeasures).

==> Makefile <==

LATEX=latex

BIBTEX=bibtex
BIBFILE=zhao.bib trapdoor.bib
PAPER= trapdoor

TEXFILES = trapdoor.tex \
	intro.tex \
	back.tex \
	methodology.tex \
	design.tex \
	analysis.tex \
	eval.tex \
	counter2.tex \
	discussion.tex \
	appendix.tex
	
EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

# $(PAPER).pdf: $(PAPER).dvi
# 	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> advance.tex <==
\section{Exploring Trapdoor Properties}

In this
section, we study the effect of injecting multiple trapdoors to a single label, and then explore facets of neuron signature computation. Neuron signature properties explored
include the layer in which the signature is computed and the number of
neurons used to create the signature. 

\subsection{Multiple Trapdoors}

\label{subsec:multiple}
Adding a single trapdoor can potentially provide a unique local ``trap" for the attacker.
A natural follow-on question is whether adding multiple trapdoors to the same label can
achieve higher detection rates of adversarial inputs.
The trapdoor set $S_t$ for target label $y_t$ is a set of trapdoors,
such that adding any one of $S_t$ to any arbitrary input will make the trapdoored model classify
the input to the target label $y_t$. This is formally defined:
\begin{definition}
The trapdoor set $S_t$ of target label $y_t$, is a set that consists
 $N$ trapdoors $\{\Delta_{1}, \Delta_{2}, \Delta_{3}, ..., \Delta_{N}\}$, such that
$\forall \Delta_i \in S_t$, $\forall x \in \mathcal{X}$, $\model(x + \Delta_i) = y_t$.
\end{definition}

Intuitively, additional trapdoors provide more local optima for attackers to
fall in, and thus increase the detection success rate. However, two other
factors come into play, and push the net impact of additional trapdoors into
the negative range.

\begin{packed_enumerate}
\item \textbf{High False Positive Rate:} With multiple trapdoors, normal
  images' neuron activations are more likely to be close to one of the
  selected trapdoors by chance.  Thus, multiple trapdoors are likely to
  increase the detection false positive rate.

\item \textbf{Mixed Effects Among Trapdoors:} In a model trained with
  multiple trapdoors, an adversarial image could converge to a single
  trapdoor, a set of trapdoors, or a combination of parts of several
  trapdoors. This potentially complicates the process of matching an
  adversarial example with one specific backdoor.
\end{packed_enumerate}

To examine the influence of these factors, we evaluate the effectiveness of
introducing more than one trapdoor in our models. We look into two
methods of injecting multiple trapdoors: multiple locations and multiple
intensities.

\para{Locations of Multiple Trapdoors.} To create the trapdoor set, we vary the
locations of trapdoors but keep intensity and shape fixed. We randomly
choose a set of $N$ locations on the image, and create the same trapdoor ($6$
by $6$ square) at each location. The set of $N$ trapdoors is the trapdoor
set of a targeted label. We trained several \gtsrb{} models, varying $N$ from
$2$ to $20$. Figure~\ref{fig:multi_loc} shows the detection success rate of
each model at $5\%$ FPR. In all cases, detection success rates are
$>75.40\%$ at $5\%$ FPR. From Figure~\ref{fig:multi_loc}, multiple location
trapdoors seem to have a negative impact on our detection
performance.

\para{Intensities of Multiple Trapdoors.} Similar to the single trapdoor analysis, we explore the trapdoors with fixed
locations but different intensities. We fix the location of a $6$ by
$6$ trapdoor at the
bottom right corner of each trapdoor injected image. We vary the trapdoors' color
intensity by sampling a different pixel intensity from a random
uniform distribution for each of the N
trapdoors. The resultant set of $N$ trapdoors is a trapdoor set for a
targeted label. We vary $N$ from $2$ to $20$. Figure~\ref{fig:multi_int}
shows the detection success rate at $5\%$ FPR. In all cases, the detection
success rate is $>88.02\%$. From Figure~\ref{fig:multi_int}, multiple
intensity trapdoors also do not seem to have a significant impact on our
detection performance. Although using multiple trapdoors to defend a
single label does not increase our detection success rate, this method
does have other interesting effects on the model that can be used
against certain adversarial countermeasures. These effects and their
use are discussed in Section~\ref{sec:counter}.

\label{sec:advance}
\begin{figure*}[t]
\vspace{-0.1in}
\centering
\begin{minipage}{0.31\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{plots/advance/gtsrb_location.eps}
  \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when injecting a number of trapdoors with different locations in \gtsrb{}.}
  \label{fig:multi_loc}
\end{minipage}
\hfill
\begin{minipage}{0.31\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{plots/advance/gtsrb_color.eps}
  \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when injecting a number of trapdoors with different intensity in \gtsrb{}.}
  \label{fig:multi_int}
\end{minipage}
\hfill
\begin{minipage}{0.31\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{plots/advance/gtsrb_check.eps}
  \caption{Detection success rate of \cw{} attack at $5\%$ FPR when using different layers for detection in a \gtsrb{} model.}
  \label{fig:change_layer}
\end{minipage}

\vspace{-0.1in}
\end{figure*}


\subsection{Measurement of Detection}
\label{sec:neurons}


Finally, we briefly investigate alternative methods of neuron
signature computation and their impacts on adversarial example
detection rates. Recall that, in our method, we use the neuron
activation pattern of a selected internal layer of the model to
compute a neuron signature for given model input. This signature is
then compared to known trapdoor signatures to determine if the input
is an adversarial example.

Several facets of the neuron signature computation -- such as the
layer chosen and the number of neurons used -- may impact our
success in detecting adversarial examples. We first explore how layer
choice impacts detection success. Figure~\ref{fig:change_layer} in the
Appendix shows the detection success rate when using different layers
of the \gtsrb{} model to compute neuron signatures. Except for the
first two convolutional layers, all later layers lead to a $>96.20\%$
detection success rate at $5\%$ FPR. We believe that neurons from
earlier layers are less useful for detection because these early
layers deal more with raw input features. However, trapdoor features
are input-independent, so they will be detected in layers deeper in
the model.


Next, we study how the number of neurons used in the signature impacts
the detection success rate. We concatenate all neurons from \gtsrb{} model, excluding the ones in the first two layers, into one vector. Then, we uniformly sample increasing percentages of
neurons ($1\%$,$2\%$...$100\%$) from the vector. For each percentage level, we use the selected set of neurons to perform our
detection. The detection success rate is $>96\%$
when more than $6\%$ of neurons are selected. This
indicates that only a small portion of the neurons is needed to create a
signature that allows detection of adversarial examples. This is good
news for the defender, giving them greater ability to avoid adaptive
attacks discussed in Section~\ref{sec:counter} if they randomly select
the neurons used for detection, \eg{randomly select $10\%$ neurons at
run time}. This prevents attackers from targeting specific neurons to avoid detection.


% \subsection{Location of the Trapdoor}

% \fixme{Is this useful to be included? -Shawn. }

% So far our injected trapdoors are mostly single squares at the bottom right corner of the images.
% There is an infinite number of possible trapdoor locations and shape. It is impossible for us to
% examine each one of them, so we will focus on several representative ones. As shown in Figure~\ref{fig:ninepoints}, We identify $9$ important points of an image, $4$ corners, the $4$ middle points of each side, and the center. We construct our trapdoors by adding a $4$ by $4$ square to a selected set of the $9$ important points, details locations follow 1. each of the $9$ points, 2. the $4$ corners, 3. the frame of $8$ on the sides, 4. all $9$ points. With the same set up as Section 4.1, we trained our models with designed trapdoors and evaluate the detection performance. At $5\%$ FPR, the detection success rate is \fixme{$>90\%$}, \fixme{$>90\%$}, \fixme{$>90\%$} for \cw{}, \pgd{} and \en{} respectively.


% Having presented the experimental success of our defense in the most
% basic context, we now evaluate more sophisticated deployments of the
% trapdoor defense. In particular, we conduct experiments to answer the
% following questions:

% \begin{itemize}
% \item Can a trapdoored model defend against untargeted adversarial
%   attacks?
% \item Can a trapdoored model defend against black box attacks?
% \item Does injecting multiple trapdoors for each defended label
%   improve our ability to detect adversarial examples?
% \item Would alternative detection metrics (i.e. different from the
%   cosine similiarity metric of Equation
%   \ref{eq:attackertrap}) increase our ability to detect adversarial
%   inputs while maintaining a low false positive rate?
% \end{itemize}

% The following paragraphs will briefly describe experiments addressing
% these questions, respectively. For each question, we produce an
% experimental ``yes'', which further confirms the effectiveness of the
% trapdoor method in defending models against adversarial attack.

% % Multiple trapdoors

% \para{Defending with multiple trapdoors per label}

% As discussed in section~\ref{sec:methodology}, a single trapdoor is an
% embedded local optimal for attacks. However, in several scenarios,
% using a single trapdoor to defend a label against adversarial attack
% may not be sufficient. In some cases, the attackers do
% not converge to the single trapdoor we provided. In a more worrisome
% scenario, attackers may be aware of the trapdoor defense employed,
% perhaps by observing patterns in the adversarial perturbation they
% create. Creating multiple trapdoors per label would, ideally, prevent
% both scenarios by providing more trapdoors for the attacker to
% converge to and by ensuring that an attacker cannot simply evade
% detection by avoiding a single trapdoor perturbation.

% To test this hypothesis, we evaluate the robustness of
% detection when multiple trapdoors are injected into a single
% label. Figure~\ref{fig:multitrap} shows the detection AUC with a
% different number of trapdoors injected per label.



% \begin{figure*}[t]
% \centering
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/placeholder.eps}
%   \vspace{-0.25in}
%   \caption{Detection AUC when different numbers of trapdoors injected per label. }
%   \label{fig:multitrap}
% \end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/untargeted_gtsrb.eps}
%   \vspace{-0.25in}
%   \caption{Defend against untargeted attack: detection success rate of adversarial image detection when achieving different false positive rate.}
%   \label{fig:untargeted}
% \end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/placeholder.eps}
%   \vspace{-0.25in}
%   \caption{Defend against black box untargeted attack: detection success rate of adversarial image detection when achieving different false positive rate.}
%   \label{fig:blackbox}
% \end{minipage}
% \end{figure*}


%% The model cannot learn the trapdoor distribution $4$ x $4$, the model fails to learn the trapdoor distribution,
%% and detection fails completely.
%% In contrast, when the length of each side
%% increases to $30$, the trapdoor is too large to trap the attacker. However,
%% there is a large middle ground between side length of $4$ to $30$, where the
%% size of the trapdoor does not have a significant impact on the detection
%% success rate. Detection success rate remains above $80\%$ for all attacks in
%% the middle region.

%\explain{This section is about pixel intensity and mask ratio. }


% In Figure\ref{fig:N} \fixme{still working on the result} shows the detection success rate at $5\%$ FPR and also the $95\%$ confidence interval.

% Before evaluating the success of the strongest adaptive attacker, we
% first examine how randomly selecting neurons in the target layer to
% compute the neuron signature impacts our detection results. For the
% \gtsrb{} model, we randomly sample $20\%$ of neurons in the target
% layer and use these to perform similarity matching. The detection
% success rate for this neuron count (at $5\%$ FPR) has a $95\%$
% confidence interval of $95.53\%$ to $96.84\%$. \emily{This next
% sentence is unclear. Do you mean to say that the detection success
% rate when we use all neurons in one layer is $96.30\%$?} The $96.30\%$ detection success rate when choosing one layer lies inside the confidence interval.

% \emily{It's a little unclear to me -- in this section you are sampling
% different percentages of neurons from the SAME layer, or different
% percentages of neurons across all layers? I'm assuming the former, but
% in that case, do you sample these different percentages across each
% layer just to see if there are any interaction effects between the
% layer used and the percent of neurons used?}

% The slightly poorly trained models results in a small drop of detection success rate, when we inject $>90\%$ of clean images with trapdoors.




% \secspace{}
% \subsubsecspace{}
% \subsection{Measurement of the Trapdoor}
% \label{sec:norm}
% \subsubsecspace{}
% The magnitude of the trapdoor $Tr_t$ forces a tradeoff between ease of injection and
% likelihood of ``trapping'' adversaries. On one hand, we wish to inject
% trapdoors that are as small as possible, because the attacker's objective is
% to minimize the attack perturbation and thus it is easier for them to converge to small
% trapdoors. On the other hand, if the trapdoor is too small, it is hard for
% the model to learn the trapdoor distribution during the injection. Here, we
% empirically examine this trade-off in the context of defending a single label. We study two ways of changing the $L2$ norm of the
% trapdoor: varying the size and the mask ratio of the trapdoor.

% \para{Size of the Trapdoor.}  We defend several \gtsrb{} models by injecting
% trapdoors of different sizes. The trapdoors are all squares at the
% bottom right corner of the image with a mask ratio $\kappa$ = $0.1$. We
% linearly increase trapdoor size from $2\text{ x }2$ pixels to
% $32\text{ x }32$ pixels (entire
% image). Figure~\ref{fig:sizetrap} shows the detection success rate (at
% $5\%$ FPR) observed in trapdoored models with trapdoors of different sizes. Trapdoors smaller than $4\text{ x }4$ or larger than $30 \text{
%   x }30$ cause detection to fail. However, for trapdoor sizes
% between these two extremes, the detection success rate remains above
% $80\%$ for all attacks. The size of trapdoor has minimal impact on normal classification
% accuracy.

% \para{Mask Ratio.} Similarly,
% we study the impact of the mask ratio $\kappa$ on the effectiveness of
% our defense. We fix the trapdoor as a $6$ by $6$ square at the
% bottom right corner and vary the mask ratio $k$ from $0.05$ to
% $1.0$. The mask ratio hugely impacts the trapdoor color intensity,
% which in turn correlates with the amount of perturbation added to the
% original image, as shown in Equation~\ref{eq:trigger}.

% We test the defense effectiveness of trapdoors with different mask ratios. Figure~\ref{fig:masktrap} shows
% detection rate at $5\%$ FPR for each model tested against our three
% attacks. As expected, detection success rate drops as the mask
% ratio of trapdoor increases. However, for reasonably small mask ratios
% ($<0.3$), detection success rate is high ($>83.34\%$ at $5\%$ FPR) and
% again minimal impact on normal classification accuracy.

% \begin{figure*}[t]
% \centering
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/gtsrb_size.eps}
%   \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when increasing the size of the injected trapdoor in \gtsrb{}.}
%   \label{fig:sizetrap}
% \end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/gtsrb_mask.eps}
%   \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when increasing the mask ratio of the injected trapdoor in \gtsrb{}.}
%   \label{fig:masktrap}
% \end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/gtsrb_rdloc.eps}
%   \caption{Detection success rate distribution of various adversarial attacks at $5\%$ FPR with differently located trapdoors. Box plot shows min/max and quartiles. \fixme{Possibly drop this to appendix. }}
%   \label{fig:distriloc}
% \end{minipage}
% \end{figure*}


% \secspace{}
% \subsubsecspace{}
% \subsection{Location of the Trapdoor}
% \subsubsecspace{}
% The location of the trapdoor could potentially impact our defense performance
% as well. For example, injecting trapdoors at locations that are critical to
% classification of normal inputs (\ie at the center or the corner of
% a traffic sign) may impact the model differently than would trapdoors
% placed elsewhere.  We choose $50$ random locations to place a
% $6\text{ x }6$ trapdoor with mask ratio $\kappa$ = 0.1, on an image. We train a defended model for
% each trapdoor location. Figure~\ref{fig:distriloc} shows the detection success
% rate distribution at $5\%$ FPR of each model. All of the detection success rates
% are above $80\%$. The location of the trapdoor does not have a
% significant impact on the detection success rate or the normal
% classification accuracy.

% \secspace{}
% \subsubsecspace{}
% \subsection{Injection Ratio}
% \subsubsecspace{}
% \label{sec:inject}
% Similarly, the number of trapdoor images we used to train the model could impact the robustness of
% the trapdoor. We call the percent of trapdoored images present in the
% training dataset the trapdoor {\em injection ratio}. More trapdoor training images could allow the model to
% learn the trapdoor better but could negatively affect normal classification accuracy. %% In Section~\ref{sec:exp}, we used $10\%$ images to be added trapdoors
% %% for the single label defense and used $50\%$ of data across all labels for the all label defense.
% We explore the impact of the injection ratio on the detection success rate and the normal classification accuracy.

% We defend several models with different trapdoor injection ratios and
% report the detection success rate in
% Figure~\ref{fig:injectratio}. When the injection ratio is less than
% $3\%$, the model fails to learn the trapdoor and therefore detection
% fails. As the injection ratio increases, the normal classification
% accuracy slowly decreases (a total of $2.75\%$), as shown in
% Figure~\ref{fig:normal_acc} in Appendix. Consequently, the injection ratio must be
% carefully chosen to ensure an ideal balance between detection success
% and normal classification accuracy.

% \begin{figure*}[t]
% \centering
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/gtsrb_inject_ratio.eps}
%   \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when increasing the injection ratio of the injected trapdoor in \gtsrb{}.}
%   \label{fig:injectratio}
% \end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/gtsrb_location.eps}
%   \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when injecting a number of trapdoors with different locations in \gtsrb{}.}
%   \label{fig:multi_loc}
% \end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{plots/advance/gtsrb_color.eps}
%   \caption{Detection success rate of various adversarial attacks at $5\%$ FPR when injecting a number of trapdoors with different intensity in \gtsrb{}.}
%   \label{fig:multi_int}
% \end{minipage}

% \end{figure*}



==> theory.tex <==
\section{Theory}
\subsection{Main Theory}

\subsection{Emily's Theory}
\begin{claim}
Consider a model $F$, with embedded trapdoor $\Delta$ for target
label $y_t$. This means that an input $x + \Delta$ has minimal loss
on the target label $y_t$, $\min \ell_F(x + \Delta, y_t)$.

An adversarial perturbation $\delta_0$ for a particular input $x_0$, targeted at label
$y_t$, will have an identical {\bf loss-space} representation as $\Delta$ (i.e. $\delta \approx
\Delta$) if $x_0 + \delta$ also has minimal loss on the target label,
$\min \ell_F(x_0 + \delta, y_t)$.
\end{claim}

\para{Proof of Claim 1}

An embedded trapdoor $\Delta$ in a model $F$ is a universal
loss-minimizing perturbation that results in misclassification to the
target label $y_t$. This means that the loss for $x + \Delta$ on the
target label $y_t$ is smaller than the loss of $x + \Delta$ on all
other labels $y \in Y$, i.e.

\begin{equation}
  F(x + \Delta) = y_t \forall x \implies \ell_F(x + \Delta, y_t) =
  \min_{y \in Y} \ell_F(x + \Delta, y)
\end{equation}

An adversarial perturbation $\delta_0$, constructed against $F$, is a
loss-minimizing perturbation for a particular input $x_0$ that causes
misclassification to the target label $y_t$. This means that the loss
of $x_0 + \delta_0$ on the target label $y_t$ is smaller than the loss
of $x_0 + \delta_0$ on all other labels $y \in Y$, i.e.

\begin{equation}
  F(x_0 + \delta_0) = y_t \implies \ell_F(x_0 + \delta_0, y_t) =
  \min_{y \in Y} \ell_F(x_0 + \delta_0, y)
\end{equation}

Since $\Delta$ is a universal trapdoor, we know that $F(x_0 + \Delta)
= y_t$. We now examine the loss functions $\ell_F(x_0 +
\Delta)$ and $\ell_F(x_0 + \delta_0)$.

To isolate the effect of $\delta_0$ and $\Delta$ on $\ell_F$, we
calculate the Taylor Series expansion of $\ell_F$ with the LaGrange
remainder. Recall that the Taylor Series expansion says that $f(x + h)
= f(x) + hf'(x) + \ldots$. With this, we have:

\begin{align*}
  \label{eq:loss_equivalence}
  \ell_F(x_0 + \Delta, y_t) &= \ell_F(x_0, y_t) + \Delta \nabla
  \ell_F(x_0, y_t) + \frac{1}{2}\zeta^T {\bf H_F} \zeta' \\
  \ell_F(x_0 + \delta_0, y_t) &= \ell_F(x_0, y_t) + \delta_0 \nabla
  \ell_F(x_0, y_t) + \frac{1}{2}\zeta^T {\bf H_F} \zeta' \\
\end{align*}

Notice that these expansions are nearly identical with the exception
of the $\Delta$ and $\delta_0$ terms. Based on this result, we can say
that if $\ell_F(x_0 + \Delta, y_t) \approx \ell_F(x_0 + \delta_0,
y_t)$, then $\ell(\Delta) \approx \ell(\delta_0)$, since all other terms cancel
out.

\begin{claim}
$\ell(x_1, y) = \ell(x_2, y) \implies G(x_1) = G(x_2)$
\end{claim}

Let $G(x)$ represent the output of the second to last layer of the model
(i.e the intermediate feature representation of the input) and $\ell(x,y)$ the loss of
the model on that input with respect the label $y$.

\fixme{FINISH THIS}

\begin{claim}
The intermediate model representation of a high-confidence adversarial perturbation $\delta_0$, constructed
against a trapdoored label $y_t$ in model $F$, must be highly similar to the
intermediate model representation of the trapdoor $\Delta$ for label $y_t$.
\end{claim}

\fixme{ This pretty much follows from the previous two claims}.

%  need to clean this up
This, of course, leaves open the question of how we ensure that
$\ell_F(x_0 + \Delta, y_t) \approx \ell_F(x_0 + \delta_0,
y_t)$. Recall that loss represents the difference between the model's
classification prediction (i.e. its relative confidence on each output
class) and the true label. If $F$ is 100\% confident about its
classification decision and is correct (i.e. it
produces the correct label $y$ for an input $x$), $\ell_F(x, y) = 0$.

Since we train the model to always classify inputs of the form $x +
\Delta$ to label $y_t$, we ensure during training time that $\ell_F(x
+ \Delta, y_t) \approx 0$.

Stronger adversarial perturbations result in more confident model
classification decisions to the target label $y_t$ and thus lower
model loss. A very strong adversarial perturbation $\delta_0$
constructed on input $x_0$ will result in the classification decision $F(x_0 +
\delta_0) = y_t$ with 100\% confidence. Furthermore, this high
confidence means that $\ell_F(x_0 + \delta_0, y_t) \approx 0$. 

Hence, an adversarial perturbation $\delta_0$ constructed on input
$x_0$ and targeted at label $y_t$ will have $\ell_F(x_0 + \delta_0,
y_t) \approx 0 \approx \ell_F(x_0 + \delta, y_t)$. By
Equation~\ref{eq:loss_equivalence}, we know this implies that
the loss-space representation of $\delta_0 \approx$ the loss space
representation of $\Delta$.

High confidence adversarial perturbations $\delta_i$ constructed against a
trapdoor-protected label $y_t$ must strongly resemble the trapdoor
$\Delta$. 

